RoboVista: Evaluating Vision Language Models for Diverse Robot Applications

Diverse applications for robotics, such as industry and agriculture, require robots to operate across various embodiments, changing visual conditions, and complex planning. Vision-Language Models (VLMs) offer a promising foundation for general-purpose and interpretable robotic reasoning. Aligning VLMs with diverse robot applications requires a modular understanding of the individual decision components that underlie robotic behavior. Capturing such structure is challenging for conventional robot benchmarks that are primarily based on teleoperated, end-to-end datasets. We propose Robot Question Answering (RQA), a modular evaluation framework and RoboVista, a benchmark curated from real robotic systems, research papers, and expert annotations. RoboVista contains 474 Visual Question Answering (VQA) instances with human annotated reasoning and covers 39 unique task types in agricultural, industrial, domestic, surgical robotics, autonomous driving, and open robot datasets. Experiments on RoboVista show that state-of-the-art VLMs exhibit substantial gaps. Physical robot experiments suggest strong correlation between RoboVista performance and real-world task execution.

==> chapters/method_old.tex <==




\section{RQA Taxonomy and Construction Method}

This section describes how we systematically construct RQA instances from robot-at-work environments using a capability-driven taxonomy. Building on the RQA definition in Sec.~\ref{def:rqa}, we introduce a structured abstraction of robot reasoning tasks, define their applicability across real-world robot domains, and formalize how human expert validation constrains question generation. Our method separates \emph{task abstraction} from \emph{domain grounding}: abstract reasoning task types are defined independently of datasets, while domain experts determine which task types can be meaningfully instantiated within a given robot-at-work environment. This design yields a principled and scalable taxonomy that supports consistent RQA construction, cross-domain evaluation, and analysis of reasoning capabilities relevant to real robotic execution.

\subsection{Robotics Tasks and Robot-at-Work Domains}

Fig.~\ref{fig:task} illustrates a capability-driven abstraction of robot-at-work systems, decomposing robot operation into functional modules commonly found in classical modular robotics pipelines. In this work, we focus on the subset of modules highlighted as solid-colored blocks, which give rise to visually grounded reasoning tasks suitable for vision–language models and robot question answering.

At the perception level, \textit{scene understanding} tasks correspond to state estimation from robot-centric observations, including geometry and spatial reasoning, sequential event understanding, and physical interaction reasoning. These tasks align with the multiview semantic correspondence, temporal understanding, and physical interaction components in Fig.~\ref{fig:task}(a), and are directly observable from visual inputs.

Building on perception, planning includes task level and motion level decision making. \textit{High-level decision making grounded on perception} captures task-level reasoning, such as goal-conditioned action reasoning, next-action or direction selection, and task sequencing. As shown in Fig.~\ref{fig:task}(b), these tasks probe how estimated state is used to select actions that advance task objectives, without requiring low-level control signals. At the execution interface, \textit{low-level motion awareness} tasks reason about action feasibility, including motion feasibility and collision avoidance, as well as closed-loop servoing guided by visual feedback (Fig.~\ref{fig:task}(c)). Finally, \textit{recovery and robustness} tasks capture failure diagnosis and recovery action selection, reflecting critical decision points during long-horizon execution (Fig.~\ref{fig:task}(d)).

We formalize this abstraction by defining a finite set of \emph{RQA task types}
$\mathcal{T}_{\text{RQA}} = \{\tau_1, \dots, \tau_{|\mathcal{T}_{\text{RQA}}|}\},$
where each task type $\tau$ represents an abstract robot reasoning capability independent of any specific dataset or robot embodiment.

Separately, we define a set of robot-at-work \emph{application domains}. Each domain $d$ corresponds to a class of real-world robot deployment scenarios, such as agriculture, industrial manipulation, domestic assistance, surgical robotics, or autonomous driving. Each domain induces characteristic sensing modalities, action spaces, and task constraints reflected in the underlying dataset $\mathcal{D}$ and task specification $\mathcal{T}$ (Def.~\ref{problem}).
\[
\mathcal{D}_{\text{dom}} = \{d_1, \dots, d_{|\mathcal{D}_{\text{dom}}|}\},
\]


This separation allows task abstractions to remain general while domains encode practical execution contexts.


\subsection{Task-Domain Mapping via Human Expert Curation}

Not all reasoning task types are meaningful in every application domain. We therefore define a \emph{task-domain applicability relation}
\[
\mathcal{M} : \mathcal{T}_{\text{RQA}} \times \mathcal{D}_{\text{dom}} \rightarrow \{0,1\},
\]
where $\mathcal{M}(\tau, d)=1$ indicates that task type $\tau$ can be meaningfully instantiated in domain $d$.

% where $(\tau, d) \in \mathcal{M}$ indicates that task type $\tau$ corresponds to a realistic and actionable reasoning requirement within domain $d$.

For each domain $d \in \mathcal{D}_{\text{dom}}$, we recruit human experts with experience in that domain to validate applicability. Experts are instructed to assess whether a task type $\tau$ can be instantiated from the robot-at-work environment $(\mathcal{D}, \mathcal{T})$ in a manner consistent with real robot sensing, control, and execution constraints. Importantly, experts are not asked to define or modify task types; rather, they determine the existence of a meaningful mapping.

This yields the domain-specific task set
\[
\mathcal{T}_{\text{RQA}}(d) := \mathcal{M}(d),
\]
which denotes the set of RQA task types applicable to domain $d$.
By construction, $\mathcal{M}$ is sparse and non-uniform, reflecting the fact that certain reasoning capabilities (e.g., closed-loop servoing) are central in some domains (e.g., surgical robotics) but irrelevant in others (e.g., agriculture robotics).


\subsection{RQA Taxonomy and Question Instantiation}

% The resulting RQA taxonomy consists of a set of abstract task types $\mathcal{T}_{\text{RQA}}$ together with a domain-conditioned task mapping $\mathcal{M}:\mathcal{D}_{\text{dom}}\rightarrow 2^{\mathcal{T}_{\text{RQA}}}$, which specifies the task types applicable to each robot-at-work domain.

Given a robot-at-work environment $(\mathcal{D}, \mathcal{T})$ associated with domain $d$, RQA instances are constructed exclusively from validated task types $\tau \in \mathcal{M}(d)$. Each RQA instance
$\mathcal{Q}_R = (\mathcal{V}, q, a^\star, \mathcal{A}, r) \in \mathbb{S}_{\text{RQA}}$
(Def.~\ref{def:rqa}) corresponds to a task-grounded decision point arising during robot execution. The visual input $\mathcal{V}$ satisfies the robot-centric constraints in Def.~\ref{def:rqa-visual}, the question $q$ probes the reasoning capability associated with task type $\tau$, and the reasoning $r$ provides algorithm- and system-grounded justification rather than generic visual description.

We denote by $\mathbb{S}_{\text{RQA}}^{(d,\tau)}$ the set of all RQA instances instantiated from domain $d$ under task type $\tau$. The full RQA benchmark is then given by
\[
\mathbb{S}_{\text{RQA}}
= \bigcup_{d \in \mathcal{D}_{\text{dom}}}
\ \bigcup_{\tau \in \mathcal{M}(d)}
\mathbb{S}_{\text{RQA}}^{(d,\tau)}.
\]
The detailed taxonomy matrix is shown in table.~\ref{tab:rqa_taxonomy_styled}

% \footnotesize
% \setlength{\tabcolsep}{4.8pt}
% \begin{tabular}{p{4.2cm} p{7.0cm} c c c c c c}
% \toprule
% \textbf{RQA Task Type} & \textbf{Description} &
% \textbf{Agri} & \textbf{Ind.} & \textbf{Open} & \textbf{Dom.} & \textbf{Surg.} & \textbf{Drive} \\
% \midrule

% \rowcolor{gray!15}\multicolumn{8}{l}{\textbf{1. Scene Understanding}} \\

% Spatial / Geometric Reasoning &
% Infer relative pose, distance, alignment, and visibility from robot-centric observations. &
% \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\

% Sequential Event Understanding &
% Reason about temporal ordering and state transitions across image or observation sequences. &
%  &  & \checkmark & \checkmark &  & \checkmark \\

% Physical Interaction Understanding &
% Infer contact, grasp state, support relations, and object motion induced by robot actions. &
% \checkmark & \checkmark & \checkmark &  & \checkmark &  \\

% \midrule
% \rowcolor{gray!15}\multicolumn{8}{l}{\textbf{2. Perception-Grounded Decision Making}} \\

% Goal-Conditioned Action Reasoning &
% Evaluate whether an action satisfies task objectives and domain constraints. &
% \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\

% Next Action / Direction Selection &
% Select the next action or motion direction based on the current scene and goal. &
% \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark \\

% Task Sequencing &
% Order subtasks to accomplish a long-horizon task objective. &
%  & \checkmark &  & \checkmark &  &  \\

% \midrule
% \rowcolor{gray!15}\multicolumn{8}{l}{\textbf{3. Motion Awareness \& Control Interface}} \\

% Motion Feasibility / Collision Awareness &
% Assess reachability, clearance, and safety constraints before execution. &
% \checkmark & \checkmark &  & \checkmark &  & \checkmark \\

% Closed-Loop Servoing &
% Reason about incremental corrections using visual feedback during manipulation. &
%  & \checkmark &  &  & \checkmark &  \\

% \midrule
% \rowcolor{gray!15}\multicolumn{8}{l}{\textbf{4. Recovery, Replanning, and Robustness}} \\

% Failure Diagnosis &
% Identify execution failures or deviations from expected task behavior. &
% \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark \\

% Recovery Action Selection &
% Select corrective actions or alternative strategies to recover task execution. &
% \checkmark & \checkmark &  &  & \checkmark &  \\

% \bottomrule
% \end{tabular}
% \end{table*}

==> chapters/problem.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{image/Robotics-pipeline.png}
    \caption{\textbf{Capability-driven abstraction of robot-at-work pipelines underlying the RQA taxonomy}.
The figure illustrates a modular view of real-world robot systems, spanning diverse application scenes and robot embodiments. Robot operation can be decomposed into four functional layers: (a) Perception / Scene Understanding, where a state estimator infers spatial, temporal, and physical interaction cues from robot-centric observations; (b) High-level Decision Making, where a meta-policy selects task sequences, plans, and discrete actions (e.g., pointing or direction); (c) Motion / Action Estimation, which evaluates motion feasibility, collision constraints, and goal reachability before execution; and (d) Failure Recovery, where system confidence, failure detection, and recovery plans close the loop. This abstraction motivates the RQA task taxonomy by aligning question types with core reasoning modules shared across robot-at-work domains.}
    \label{fig:task}
\end{figure*}


\section{Problem Formulation}
\subsection{RQA Definition}
We first define a general multiple-choice VQA instance with reasoning, then define RQA as a robot-centric subset of the general VQA set.

\begin{Def}{(VQA Instance with Reasoning)}
\label{def:vqa}
Let $\mathbb{V}$ denote the space of admissible visual inputs (single image, multi-image, or short video clip), and
let $\mathbb{Q}$ be the space of natural-language questions, $\mathbb{A}$ the space of candidate answers, and $\mathbb{R}$ the space of textual rationales.
A VQA instance with reasoning is a 5-tuple
\[
\mathcal{Q} = \left(\mathcal{V},\; q,\; a^\star,\; \mathcal{A},\; r\right)\in
\mathbb{V}\times\mathbb{Q}\times\mathbb{A}\times 2^{\mathbb{A}}\times\mathbb{R},
\]
where $\mathcal{V}\in\mathbb{V}$ is the visual input, $q\in\mathbb{Q}$ is the question, $a^\star\in\mathbb{A}$ is the ground-truth answer,
$\mathcal{A}\subseteq\mathbb{A}$ is a finite set of multiple-choice candidates with $a^\star\in\mathcal{A}$, and
$r\in\mathbb{R}$ is the reasoning that justifies $a^\star$ (and may explain why distractors are incorrect).
We denote the set of all such instances by
\[
\mathbb{S}_{\text{VQA}} := \mathbb{V}\times\mathbb{Q}\times\mathbb{A}\times 2^{\mathbb{A}}\times\mathbb{R}.
\]
\end{Def}

\begin{Def}{(Robot-Centric Visual Input)}\label{def:rqa-visual}
Define two robot-centric constraint subsets of 
$\mathbb{V}$:
\begin{align*}
    \mathbb{V}_{\text{rv}} &:= \{\mathcal{V}\in\mathbb{V}:\mathrm{RobotVisible}(\mathcal{V})\}, \\
\mathbb{V}_{\text{ob}} &:= \{\mathcal{V}\in\mathbb{V}:\mathrm{Onboard}(\mathcal{V})\},
\end{align*}
where $\mathrm{RobotVisible}(\mathcal{V})$ indicates the robot is clearly visible in $\mathcal{V}$, and
$\mathrm{Onboard}(\mathcal{V})$ indicates $\mathcal{V}$ is captured by onboard sensors during execution.
\end{Def}

\begin{Def}{(RQA Instance)}
\label{def:rqa}
RQA is the subset of VQA instances with reasoning whose visual input is robot-centric:
\[
\mathbb{S}_{\text{RQA}}
:= \left\{\mathcal{Q}=(\mathcal{V},q,a^\star,\mathcal{A},r)\in \mathbb{S}_{\text{VQA}}
\;:\; \mathcal{V}\in \mathbb{V}_{\text{rv}} \cup \mathbb{V}_{\text{ob}}\right\}.
\]
Any $\mathcal{Q}\in\mathbb{S}_{\text{RQA}}$ is called an \emph{RQA instance}.
\end{Def}



\subsection{Problem Definition}

We consider the problem of constructing robot-centric visual question answering instances from robot-at-work environments. A robot-at-work environment is specified by a pair $(\mathcal{D}, \mathcal{T})$, where $\mathcal{D}$ denotes a robot dataset and $\mathcal{T}$ denotes the corresponding robot task specification.

A robot dataset $\mathcal{D}$ may vary widely in scope, sensing configuration, and application domain. Nevertheless, its contents can typically be organized into three components: (i) multi-modal sensor streams collected during task execution, (ii) semantic annotations describing objects, actions, or outcomes, and (iii) system metadata that specifies the robot embodiment, sensors, and data-collection platform~\cite{Robo2VLM-journal}. The task specification $\mathcal{T}$ captures the intended robot behavior, including task objectives, operational constraints, success criteria, and, when applicable, decision logic governing task execution.

\begin{Pro}[RQA Construction from Robot-at-Work Environments]
\label{problem}
Given a robot-at-work environment specified by $(\mathcal{D}, \mathcal{T})$, the RQA construction problem is to generate a robot-centric visual question answering instance
\[
\Phi:\; (\mathcal{D}, \mathcal{T}) \;\longrightarrow\; 
\mathcal{Q}_R = (\mathcal{V}, q, a^\star, \mathcal{A}, r) \in \mathbb{S}_{\text{RQA}},
\]
where $\mathcal{Q}_R$ represents a single task-grounded decision point arising during robot execution.
\end{Pro}

The constructed visual input $\mathcal{V}$ must satisfy the robot-centric constraints defined in Def.~\ref{def:rqa-visual}, ensuring that the robot is either visible in the scene or that the observation is captured by onboard sensors during task execution. The remaining elements $(q, a^\star, \mathcal{A}, r)$ encode a well-posed decision or reasoning query grounded in the task specification $\mathcal{T}$. In particular, $\mathcal{A}$ denotes a finite set of challenging yet unambiguous answer choices with a unique correct answer $a^\star$, and $r$ provides algorithm- and system-grounded reasoning that justifies $a^\star$ while ruling out distractors.

==> introduction.tex <==



\section{Introduction}
%  A natural choice for VLM is to anwser 
% with challenge of human labeling, homogeneity, simulation etc. 
% open x (existing ) make it possible
%in this paper, we present a system maethod for generating large and high quality VQA benchmark from heten human-curated and teleoperated robot demonstration 

% embodied reasoning 

% need to introduce the robot space relationshp, understanding why it's the case, then VLM is there to help with assumption that VLM can infuse real world knowlege. this ability is assumed, but hardly studied systematically.
% Humans naturally exhibit sophisticated intelligence in manipulation—the ability to perceive complex scenes, understand spatial relationships, and plan physical interactions with the target object—a capability fundamental to tasks ranging from simple grasping to intricate tool manipulation.
% Replicating this ability is crucial for advancing robotic manipulation. 
% These applications typically operate under the assumption that VLMs have inherently learned this capability during pre-training.

% Humans naturally exhibit sophisticated intelligence in manipulation—the ability to perceive complex scenes, understand spatial relationships, and plan physical interactions with the target object—a capability fundamental to tasks ranging from simple grasping to intricate tool manipulation.
Emerging Vision-Language Models (VLMs)~\cite{radford2021learning,qwen2.5,liu2023visual,anthropic2024claude35,openai2024gpt4o,google2025gemini25} can perform high-level reasoning and scene interpretation~\cite{Chen_2024_CVPR,karamcheti2024prismatic} for robots.
Recent robotic manipulation systems that integrate VLMs demonstrate enhanced capabilities in semantic and long horizon task reasoning \citep{kim24openvla,geminiroboticsteam2025geminiroboticsbringingai,shi2025hirobotopenendedinstruction}.
Yet, a key challenge persists: the image-text corpora used for VLM pre-training lacks fine-grained spatial and task information, which are prerequisites for robots to identify  complex scenes, reason about spatial relationships, and plan physical interactions.


To address this challenge, some research relies on data generation through simulation~\cite{islam2024eqamx, yang2025embodiedbench, li2024eai, shridhar2020alfred, szot2021habitat, kolve2017ai2thor}.
However, simulators cannot accurately model physical properties such as contact dynamics, and interactions. Therefore, strong performance in simulation often fails to translate reliably to the physical world.
Meanwhile, deriving spatial knowledge from real-world data typically requires extensive and costly human labeling~\cite{sermanet2023robovqa,ji2025robobrain}.
In contrast, teleoperated robot demonstration that are used to train visuomotor policies~\cite{levine2016end}, such as Vision-Language-Action (VLA)~\cite{kim24openvla,octo_2023} or diffusion policies~\cite{chi2023diffusionpolicy}, typically include multiple images from different cameras, precise proprioceptive and kinematic information, such as joint angles, end-effector poses, gripper states, and force–torque readings, that implicitly encode 3D spatial information. We hypothesize that, given such datasets, we can extract visual and textual data to improve VLM's spatial and task reasoning capabilities. 

We present \benchname, a multiple-choice Visual Question Answering (VQA) dataset generation framework (Fig.~\ref{fig:title}). Given a human-teleoperated robot demonstration, \benchname uses 
human annotation and data modalities, such as gripper aperture, to segments the demonstration and select image frames. 
\benchname generates questions whose answers are supported by synchronized proprioceptive and kinematic ground truth.
We apply \benchname to 276k diverse, real-world demonstration from the Open X-Embodiment (OXE) dataset~\cite{open_x_embodiment_rt_x_2023} crowdsourced from research labs worldwide and Agibot~\cite{bu2025agibot_arxiv} dataset that contain dense task annotations. 
We generate 864,753 VQA samples, covering 463 distinct scenes, 3,396 robotic manipulation tasks, and 149 manipulation skills.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/Screenshot 2025-11-30 at 9.00.47 PM.png}
    \caption{\textbf{Robo2VLM} transforms real teleoperated robot demonstration that contain observations, semantic labels, and system metadata into structured visual questions through template prototyping, visual augmentation, answer derivation, and question curation. The resulting VQA dataset enables post-training and evaluation of modern Vision-Language Models onstate, action, causal, goal-conditioned, and interaction reasoning}
    \label{fig:title}
\end{figure}

%  

 % We comprehensively evaluate state-of-the-art multimodal models on HourVideo (Tab. 2, Fig. 4), including GPT-4V [2], Gemini 1.5 Pro [3], and LLaVA-NeXT [ 14 ] in a zero-shot setting. Our findings reveal that GPT-4V and LLaVA-NeXT achieve only marginal improvements over a random predictor (20\%), obtaining accuracies of 25.7\% and 22.3\%, respectively. Gemini 1.5 Pro, designed specifically for long-context multimodal understanding, obtains an accuracy of 37.3\%, which, while better, is still substantially lower than the average performance of human experts at 85.0\%. 

% We distill \dsname to a 50k training set and 10k testing set. 
% Using \dsname training set to 
% \begin{comment}
We validate with human annotator a 4,000 question subset of \dsname as the testing set.
We evaluate state-of-the-art open source models (Llama, Gemma and Qwen) and with different parameter sizes. The results indicate that some VLMs can achieve near human performance in scene understanding questions, such as object reachability and interaction understanding. Evaluation data also suggests that prompt with thinking improves questions that require temporal and task reasoning, such as identifying the goal configuration of a task. 
However, results suggest that smaller models and categories directly relating to perception lead to overthinking~\cite{lithink} and compromise the performance.

To study how Robo2VLM improves VLM performance, 
we use Supervised Finetuning (SFT)~\cite{ouyang2022training} to finetune Qwen2.5-VL~\cite{qwen2.5} with \dsname. We evaluate the finetuned model with \dsname-Bench and Embodied Reasoning Question Answering (ERQA) benchmark~\cite{geminiroboticsteam2025geminiroboticsbringingai}, a state-of-the-art benchmark curated by Google DeepMind for Gemini Robotics models~\cite{team2025gemini} and has become a widely adopted measure of spatial understanding and embodied reasoning in VLMs, including Qwen3~\cite{yang2025qwen3}. Evaluation data shows finetuning with \dsname improves the spatial and interaction understanding on \dsname-Bench. The improvement is transferable up to a 6.2\% accuracy gain on ERQA.
% Such a gain highlights that the benefits of our dataset extend well beyond its training domain and meaningfully strengthen general-purpose embodied reasoning.
% By fine-tuning on \dsname with different training dataset size on LLaVA 1.6, we show  substantial improvements across most VQA categories, such as understanding task state. \eric{need to include numbers}

This paper makes the following contributions: 
(1) \benchname, a VQA data generation framework from robot demonstration datasets
(2) \dsname, an open VQA dataset with 864,753 questions covering diverse and realistic evaluation scenarios for manipulation. 
(3) Evaluation data on open-source VLMs and fine-tuned VLMs.





% \end{comment}
